Integrated Radio Sensing Capabilities for 6G Networks: AI/ML Perspective

The sixth-generation wireless communications (6G) is often labeled as "connected intelligence". Radio sensing, aligned with machine learning (ML) and artificial intelligence (AI), promises, among other benefits, breakthroughs in the system's ability to perceive the environment and effectively utilize this awareness. This article offers a tutorial-style survey of AI and ML approaches to enhance the sensing capabilities of next-generation wireless networks. To this end, while staying in the framework of integrated sensing and communication (ISAC), we expand the term "sensing" from radar, via spectrum sensing, to miscellaneous applications of radio sensing like non-cooperative transmitter localization. We formulate the problems, explain the state-of-the-art approaches, and detail AI-based techniques to tackle various objectives in the context of wireless sensing. We discuss the advantages, enablers, and challenges of integrating various sensing capabilities into an envisioned AI-powered multimodal multi-task network. In addition to the tutorial-style core of this work based on direct authors' involvement in 6G research problems, we review the related literature, and provide both a good start for those entering this field of research, and a topical overview for a general reader with a background in wireless communications

==> figures/isic_general_spatial.tex <==
\begin{tikzpicture}
%\pic[color=KITgreen, fill=KITgreen, scale=0.4] (car1) at (2,-2) {car};
\node[black, circle, radius=0.7cm,label={[yshift=-0.25cm]below:Objects}] (car1) at (3,-1) {};
%\node[black, circle, radius=1cm,label=below:Objects] (car2) at (3,0) {};
%\pic[fill=black!80!white, scale=0.3] (car2) at (4.5,-1.3) {car};
%\pic[fill=KITpurple, scale=0.3, xscale=-1] (car3) at (5.5,-3) {car};

\shade[ball color = gray!40, opacity = 0.4] (3,0.5) circle (0.2cm);
\node (d) at (3,0){\vdots};
\shade[ball color = gray!40, opacity = 0.4] (3,-1) circle (0.5cm);
\pic[thick, scale=0.2, color=black!60!white] (BS1) at (1,0) {MBS};
\pic[thick, scale=0.2, color=black!60!white] (BS2) at (5,0) {MBS};
\pic[thick, fill=white, scale=0.2] (UE1) at (-0.5,-0.5) {phone};

\draw [decoration={expanding waves,angle=10,segment length=2mm},decorate,draw,color=black] (BS1-a1) -- ($0.5*(UE1-base)+0.5*(BS1-a1)$);% node[midway, label={[yshift=7mm,xshift=-15mm]above:\small{communication}}] {};
\draw [decoration={expanding waves,angle=10,segment length=2mm},decorate,draw,color=black](BS1-a2) -- ($0.5*(car1)+0.5*(BS1-a2)$);% node[midway, label={[yshift=7.5mm,xshift=15mm]above:\small{sensing}}] {};

\draw [decoration={expanding waves,angle=6,segment length=2mm},decorate,draw,color=black!40, thick](car1.north) -- ($0.3*(d.south)+0.7*(BS2-a1)$);
%\draw [decoration={expanding waves,angle=4,segment length=2mm},decorate,draw,color=black!40,thick](car2-base) -- ($0.5*(car2-base)+0.5*(BS1-base)+(0,0.5)$);
%\draw [decoration={expanding waves,angle=4,segment length=2mm},decorate,draw,color=black!40, thick](car3-base) -- ($0.5*(car3-base)+0.5*(BS1-base)+(0,0.5)$);

\begin{scope}[on background layer={color=KITgreen!10}]
    \fill (-1,-2) rectangle (1,1.5);
    \node[KITgreen](a) at (0,-1.7) {\footnotesize Communication};
  \end{scope}

\begin{scope}[on background layer={color=KITpalegreen!10}]
    \fill (1,1.5) rectangle (6,-2);
    \node[KITpalegreen](a) at (5.4,-1.7) {\footnotesize Sensing};
  \end{scope}

\end{tikzpicture}

==> figures/overview_alt_graphic.tex <==
\tikzset{block/.style={rectangle, thick, draw, minimum width=5cm, minimum height=4cm, rounded corners=1.6mm},align=center}
\begin{tikzpicture}[>=latex]
    \matrix [nodes=draw,column sep=1cm,left color=KITblue!40, right color=KITred!40]
  {
    \node[block,fill=KITblue!40] (a) {\begin{minipage}{0.3\linewidth}
        Object detection \& Localization
    \begin{itemize}
        \item Distinguish objects of interest from clutter
        \item Estimate range, Doppler, \ac{AoA}, 2D or 3D coordinates
    \end{itemize}
    \end{minipage}}; & \node[block, fill=KITblue!50!KITred!40] {\begin{minipage}{0.3\linewidth}
        Emitter Localization
    \begin{itemize}
        \item Localization of known or cooperative transmitters using \ac{AoA}, \ac{ToA}, \ac{TDoA}
        \item Localization of unknown/non-cooperative transmitters
    \end{itemize}
    \end{minipage}};  & \node[block, fill=KITblue!20!KITred!40] {\begin{minipage}{0.3\linewidth}
        Channel Sounding
    \begin{itemize}
        \item Characterization of the radio environment
        \item Network planning
    \end{itemize}
    \end{minipage}}; & \node[block, fill=KITred!40] (b) {\begin{minipage}{0.3\linewidth}
        Spectrum Sensing:
    \begin{itemize}
        \item Detect occupancy of radio channel
        \item Detect presence of a specific user
    \end{itemize}
    \end{minipage}}; \\ [2mm]
    \node[block, fill=KITblue!40] {\begin{minipage}{0.3\linewidth}
        Object classification
    \begin{itemize}
        \item Spatial object orientation
        \item Size, micro-Doppler, distinguish between different object types
    \end{itemize}
    \end{minipage}}; &      \node[block, fill=KITblue!50!KITred!40] {\begin{minipage}{0.3\linewidth}
        Channel Charting
    \begin{itemize}
        \item \ac{UE} pseudo-positioning 
        \item UE path or channel prediction
    \end{itemize}
    \end{minipage}}; &    &    \node[block, fill=KITred!40]  {\begin{minipage}{0.3\linewidth}
        Signal Classification:
    \begin{itemize}
        \item Anomaly \& jamming detection
        \item Waveform classification
    \end{itemize}
    \end{minipage}}; \\ [2mm]
    \node[block, fill=KITblue!40] {\begin{minipage}{0.3\linewidth}
        Object tracking
    \begin{itemize}
        \item Combine multiple measurements to reconstruct trajectory
        \item Estimate range, Doppler, \ac{AoA}, 2D or 3D coordinates
    \end{itemize}
    \end{minipage}}; &       &        & \\
  };
   \draw [<->,KITred,thick] ($(a.west)+(0,2.5)$) -- ($(b.east)+(0,2.5)$) node [above,near start] {\Large \textcolor{KITblue}{Spatial Sensing}} node [above,near end] {\Large Spectrum Sensing};
\end{tikzpicture}


==> tex_files/ISAC_est.tex <==
\newcommand{\jose}[1]{\textcolor{blue}{\footnotesize{\textsf {[Jose: #1]}}}}

\section{Spatial Sensing of Passive Objects}\label{sec:isac}
Spatial sensing in \ac{ISAC} refers to radar-like sensing performed by a node in a wireless network as generically shown in Fig. \ref{fig:isac-spatial-general}. 
A signal, that might also be used for communication, is transmitted and reflected by features of the environment. 
The reflected signal is received by the same or a different node and features of the environment can be extracted from the received signal by estimating the channel parameters of a channel model such as the ones discussed in Sec.~\ref{sec:channel-model}. 
Depending on the features to be extracted and the transmit waveform used, different signal processing and estimation methods are employed.

In this section, we demonstrate how \ac{ML} methods can be applied to improve \ac{ISAC} systems in general, addressing the interaction of communication and sensing, and shedding light on the associated computational complexity. Furthermore, we show the role \ac{ML} can play when exploring new \ac{ISAC} network paradigms. 
The remainder of the section addresses different environment parameters that can be sensed. We provide descriptions of classical solutions for the estimation problem, if applicable, and present how \ac{ML} methods can improve the sensing performance. 
We note that, in general, it is beneficial to perform a joint detection and estimation, as this always provides the optimal separation simply from more available dimensions for the separation, and hence detection, of targets.
E.g., a joint detection in range-Doppler and angle will yield better results compared to a range-only detection.
However, whether it is viable or not depends on the signal waveform, measurement hardware, and efficiency of the used signal processing, as large amounts of data must be processed jointly. 

\begin{figure}
    \centering
    \input{figures/isic_general_spatial}
    \caption{A generalized ISAC setup for spatial sensing.}
    \label{fig:isac-spatial-general}
\end{figure}

%\todo[inline]{for now: max 1 graphic per subsection (weak rule)-> kick stuff out later}
%\subsection{\ac{ISAC} optimization (Charlotte)}
\subsection{\ac{ISAC} Trade-offs}
While many challenges in \ac{ISAC} are attributed to either the communication or the sensing side, this section considers the problems unique to the combination of both, which arise either from resource sharing or communication and sensing with the same \ac{TX} signal.

Fundamentally, \ac{ISAC} systems are subject to either the deterministic trade-off and the subspace or a power trade-off~\cite{Xiong2023}. \par
The deterministic trade-off stems from the fact that the communication performance of systems is maximized if the modulation symbols are randomly distributed, but for sensing, a deterministic transmit signal is preferred. 
Specifically,for sensing, transmit symbols of equal power are optimal, which limits the communication performance.\par
The subspace or power trade-off refers to the transmit resources such as power or bandwidth being shared between sensing and communication.
In a classical system, performance can be traded off through time sharing, or other methods akin to resource allocation for multiple users. 
% Taking the information rate and the Bayesian \ac{CRB} $\epsilon$ of sensing into account, time sharing results in the trade-off
% \begin{align}
%     \epsilon = \epsilon_{\min}+\frac{\epsilon_{\max}-\epsilon_{\min}}{R_{\max}-R_{\min}} (R-R_{\min}),
% \end{align}
% while $\epsilon_{\max}$ is achieved under maximum communication throughput $R_{\max}$ of the given system and $R_{\min}$ is achieved under optimum sensing performance $\epsilon_{\min}$. This linear trade-off can represent systems with sensing in the time slots with communication signals,i.e. $\epsilon_{\max}<\infty$, or when during communication no sensing information is processed, i.e. $R_{\min}=0$.

However, there is a performance gap which is difficult to explore with rigid resource sharing methods.
\Ac{ML} can be used to explore the trade-off spaces and find good operating points that meet design criteria for both functionalities or provide adaptive operating points. Additionally, it is of interest to shed light on the synergies of both functionalities and optimize the transmit signal. 
Classical optimization methods can be computationally expensive and inflexible, whereas \ac{ML} can provide \textit{good-enough} approximations, often at low computational cost.

\begin{figure}
\centering
\includegraphics{figures/spatial_sens/power_tradeoff.pdf}
    
\includegraphics{figures/spatial_sens/deterministic_tradeoff.pdf}
    \caption{Examples how power trade-off or deterministic tradeoff can manifest in an \ac{ISAC} system from~\cite{muth2024loss} (\copyright[2024]IEEE).}
    \label{fig:isac-tradeoff}
\end{figure}

Using beamforming to show an example of the power trade-off, we can achieve synergies if the areas of interest coincide.
If sensing is performed in an area separate from the position of the communication \ac{RX}, we observe a worst-case scenario for the power trade-off.
Beamforming or precoding with a transmitter with $L$ antennas can be expressed using a far-field assumption as
\begin{align}
    s_{\text{Tx}}(t) = \sum_{\ell=0}^{L-1} w_{\ell} x_{\text{Tx}}(t-\tau_{\ell}).
\end{align}
Using complex weights $w_{\ell}$, the beampattern resulting from interference can be controlled. Using an \ac{ULA} with antenna spacing $d$ and the carrier wavelength $\lambda$, we can rewrite the expression for a transmit signal in a angular direction $\varphi$ as
\begin{align}
    s_{\text{Tx}}(t,\varphi) = \sum_{\ell=0}^{L-1} w_{\ell} x_{\text{Tx}}(t) e^{\j2\pi \ell \frac{d}{\lambda}\sin(\varphi)}.
\end{align}
In this example, the beamforming weights $w_{\ell}$ are optimized as the output of an \ac{NN} with the loss term
\begin{align}
    L(\mat{\Theta}) = (1-w_{\text{s}})\mathcal{L}_{\text{BCE}}^{\text{commun}}(\mat{\Theta}) + w_{\text{s}}\left(\mathcal{L}_{\text{BCE}}^{\text{detect}}(\mat{\Theta}) + \mathcal{L}_{\text{MSE}}^{\text{angle}}(\mat{\Theta})\right),
    \label{eq:isac-tradeoffs}
\end{align}
with the \ac{NN} parameters $(\mat{\Theta})$ and the loss terms referring to the definitions in \eqref{MSE_eq}-\eqref{BCE} applied to the tasks of communication, detection and angle estimation.
In an example scenario, shown in Fig.~\ref{fig:isac-tradeoff}, the \ac{ISAC} system detects targets in a certain area of interest, while communicating with an \ac{UE} in a different area of interest. Depending on the importance of sensing indicated by $w_{\text{s}}$, power gets transmitted more toward the sensing area or toward the communication receiver.

Multiple research groups have addressed this trade-off using \ac{ML} methods.
In~\cite{MateosRamos2021, muth2023autoencoder, muth2024loss}, static beam-patterns were trained using a \ac{DNN} in an end-to-end fashion, with the \ac{MSE} of \ac{AoA} estimation, the \ac{CE} for target detection and the \ac{MI} between \ac{TX} and \ac{RX} contributing to the loss term. The \ac{DNN} needs output normalization, as otherwise the end-to-end framework incentivizes the output power to become infinitely high. 
Additional legal output constraints of a wireless transmission are considered in~\cite{fontanesi2024deep} for beamforming in \ac{UE}-centric sensing. The chosen scenario consists of beamforming for sensing and communication with a choice of suitable base stations, leading to a generally non-convex optimization problem. A predictive beamforming approach is trained using a \ac{DNN}, using the absolute error between the targeted side lobe level and effective isotropic radiated power in the loss function.
As a last example, hybrid beamforming algorithms with multiple objectives are implemented in~\cite{Nguyen2023} using deep unfolding. A classical iterative optimizer with a fixed number of iterations is transformed into an \ac{DNN}, enabling fast convergence.

In a more general sense, the power-trade off also can manifest as a resource allocation problem. In systems where time or frequency resource blocks are allocated to either communication or sensing, the main indicator of sensing performance is the amount of resources reserved for sensing. This problem is addressed in~\cite{Yang2024a} and~\cite{Liu2025} using~ac{RL}.

Concerning the deterministic trade-off, classical solutions to find good transmit signals have been hand-designed or limited to constant-modulus transmit signals to maximize sensing performance while enabling communication. Constellation shaping is being explored as a method to set flexible deterministic trade-offs, often being implemented using a \ac{DNN} mapping the input bit to constellation symbols.  Probabilistic constellation shaping, which uses QAM constellations but attributes different probabilities to different constellation points, is used to jointly optimize communication and sensing performance, demonstrating ability to steer the deterministic trade-off in~\cite{Yang2024}. Geometric constellation shaping, where the position of constellation points is optimized, is shown in Fig.~\ref{fig:isac-tradeoff} for $16$ constellation points. For high $w_{\text{s}}$, as defined in \eqref{eq:isac-tradeoffs}, the constellation tends towards a 16-PSK and with a trade-off tending toward communication it resembles a 16-QAM. 
Constellation shaping has been analyzed in more detail in~\cite{geiger2025jointshaping} for \ac{OFDM}-\ac{ISAC} systems. It was shown analytically that constellation kurtosis is the deciding factor in possible sensing performance, independent of the used shaping method. The deterministic trade-off can therefore be flexibly used to improve either communication or sensing performance compared to classical methods. Therefore, a loss function optimizing the communication performance with an added constraint for the kurtosis can be used instead of an end-to-end evaluation of the communication and sensing performance, respectively.

Notably, many \ac{ISAC} studies do not focus on the communication functionality, although it has a significant impact on the performance of an \ac{ISAC} system if both functionalities share the same transmit resources.

%\item Signal compensation: Mitigate the sensing echo and uplink communication signal interference, using unsupervised learning \cite{qi2024deep}. Assumes that sensing echos from BS are in uplink phase (so we sense far away objects), demonstrate improvements in complexity and the application to complex optimization problems

%\begin{itemize}
    %\item OFDM structure specific compensation
    % \item Power Trade-off: Beamforming algorithms
    % \begin{itemize}
    %     \item as beamforming means power trade-off and also important for objet tracking of special interest for ISAC. ML approaches such as deep unfolding~\cite{Nguyen2023}, 
    %     \item Design of beams in THz UAV ISAC \cite{fontanesi2024deep}.
    %     \item Alternatively to the trade-off in resource allocation, we can also shift the power assigned to both functionalities, assuming the worst case that the area where communication receivers are located is not the area where sensing is to be performed. Depending on the importance of sensing $w_{\text{s}}$, different beam-patterns trading off power are shown in Fig.~\ref{fig:isac-tradeoff}
    % \end{itemize}
    %\item Deterministic Trade-off: Constellation shaping
    %\begin{itemize}
        %\item joint optimization steers the deterministic ISAC trade-off, here probabilistic constellation shaping~\cite{Yang2024}
        %\item Charlottes colleague Benedikt Geiger is just about to finish a paper on joint constellation shaping for ISAC
        %\item In Fig.~\ref{fig:isac-tradeoff}, the deterministic tradeoff for multiple observations is visualized, as the modulation constellations for an \ac{ISAC} system using the sensing symbols also for communication are shown. Depending on the tradeoff factor $w_{\text{s}}$, denoting the importance of the sensing functionality, the constellation shifts from a sensing-optimal \ac{PSK} (constant-modulus modulation) to a modulation resembling an 16-\ac{QAM}. 
    %\end{itemize}
 
%    \end{itemize}
%(Charlotte)
\subsection{Complexity Reduction}
Efforts in complexity reduction include reduction of computational complexity, simplification of data acquisition, increased flexibility of algorithms and increased accessibility of training methods. 

The computational complexity of applied algorithms in \ac{ISAC} is an important factor in the algorithm's latency, associated power consumption, and hardware requirements. Consequently, achieving similar performance while reducing complexity remains a vital direction to explore. For \ac{ML} methods, we need to differentiate between the training and inference complexity. While training is usually performed once offline, being limited only by the time and hardware resources dedicated to training, the algorithm will be run many times with inference complexity on hardware with more limited resources. Research activities for complexity reduction tend to compare different \ac{ML} solutions based on complexity that achieve similar performance. For trainable algorithms, the complexity of training and inference has to be considered separately. Complexity reduction is not unique to \ac{ISAC}, but as \ac{ISAC} algorithms are to run on cost-effective hardware with low latency it is of special interest.

% MBL section -> move to section 3
\Ac{MBL}~\cite{shlezinger2023model} merges traditional model-based signal processing with \ac{DL} parameterizes traditional model-based signal processing to overcome the limitations of conventional methods. 
For instance, given a mapping $f:\mat{D} \in \mathcal{D} \to \mat{Y} \in \mathcal{Y}$, \ac{MBL} computes the output as
\begin{equation} \label{eq:mbl}
	\mat{Y} = f(\mat{D}; \mat{\Theta}) = g \circ h (\mat{D};\mat{\Phi}) ,
\end{equation}
where $h (\mat{D};\mat{\Phi})$ is a function with learnable parameters $\mat{\Phi}$ (e.g., a NN), $g$ is a function with no learnable parameters (e.g., a conventional model-based algorithm), and $\circ$ represents the composition of functions.\footnote{The function $h (\mat{D};\mat{\Phi})$ does not be to be the first function, it can be placed and designed anywhere in the conventional algorithm.} The function $g$ must be differentiable to enable backpropagation and learning of $\mat{\Phi}$.
By incorporating domain knowledge, such as conventional receiver structures and algorithms, into the design of the \ac{NN} architecture, this approach improves interpretability while improving training and inference efficiency and reducing the amount of training data required.
Instead of training a \ac{DNN} to perform a specific task from scratch, \ac{ML} is employed to optimize the performance of existing algorithms, for example, by tuning parameters to particular channel conditions and environments.

Methods like \ac{MBL} and deep unfolding limit the amount of trainable parameters, while being able to achieve the same performance than pure \ac{ML} solutions in some scenarios~\cite{shlezinger2023model}. Choosing the algorithm structure and which parts of a classical algorithm benefit from being enhanced with trainable features is vital to achieve sleek and powerful solutions for complex problems.
In~\cite{jiang2024isac}, deep unfolding is used for bistatic joint sensing. The hyper-parameters of an \ac{ISAC} algorithm to perform range-velocity estimation and communication demodulation are optimized, and the work compares performance and complexity of this approach with other classical and trainable algorithms.

From an hardware-implementation or deployment point of view, complexity is also of importance \todo[inline]{fixme}
As an alternative \ac{ML} paradigm, spiking \acp{NN} promise increased power efficiency in combination with neuromorphic hardware. 
% Neuromorphic computing -> move to section 3
In contrast to artificial \acp{NN}, spiking \acp{NN}, have emerged as a contenting paradigm of neuromorphic computing promising higher energy efficiency. Their signal flows are designed to emulate the function of biological neurons closer than artificial \acp{NN} by processing discrete spikes, spread at arbitrary time instances, instead of floating point numbers. As biological neurons are known to be very energy efficient, emulating them closer promises complex \ac{AI} models with a fraction of the power consumption compared to current models. A neuron can have multiple inputs that contribute to the membrane potential. When the membrane potential reaches a threshold, a spike is output by the neuron and the membrane potential is reset. Therefore, certain features such as clock-less computing, an inherent memory and a promise of high energy efficiency if implemented in hardware have attracted the attention of multiple research groups. In spiking \acp{NN}, different features of these neurons are made trainable, enabling the application of different \ac{ML} training methods to these new structures.
We refer the reader to~\cite{Eshraghian2023} for a thorough introduction into spiking \acp{NN}.
In~\cite{chen2023neuromorphic}, spiking \acp{NN} are developed to perform object detection and communication demodulation in an \ac{ISAC} system. Although the paradigm shift from floating-point values to temporal spikes can be challenging, some applications such as impulse radio or pulse-based sensing can potentially be easier represented in this signal space. 

% Concerning data acquisition, methods are studied that need less training data is to converge, through i.e. \ac{MBL} or new \ac{NN} architectures. With varying availability of clean training data, robustness concerning errors in the training data can be seen as an added performance indicator. It is yet also unclear if acquisition from multiple sites or a single site are sufficient for deployable \ac{ISAC} systems.
% Although algorithms can be trained for specific sites, it might prove more efficient to enable systems to generalize. This could be implemented by training a general method before limited training with site- or scenario-specific parameters. Additionally, the paradigm of continuous learning is of interest when generalization to new environments is discussed.

% The accessibility of learning methods relates to how easily \ac{ML} can be implemented by an interested party. 
% Although many tools supporting researchers to explore \ac{ISAC} using \ac{ML} have been developed such as~\cite{Hoydis2023}, many \ac{ML} frameworks are developed from the perspective of language or image processing, imposing restrictions as mentioned in Sec.~\ref{sec:ml-basics} when simulating wireless systems.

%(Charlotte)
\subsection{System Extension}
New network paradigms can introduce a mass of new degrees of freedom. 
Especially if \ac{ML} is already employed within the system, exploring different operating points with \ac{AI} might be an accessible option for system characterization. 
With classical systems, the theoretical description of the interfaces needs to be combined, usually increasing the degrees of freedom significantly. 
The optimization for one or multiple objectives of such a system becomes very difficult. 
Using \ac{ML}, we can find solutions within given constraints for system configurations or experiment on the interactivity of different components. 
Such new paradigms include non-terrestrial networks~\cite{Matera2024}, distributed multiple-input multiple output~\cite{Wild2021,Guo2024} or extremely large-scale antenna arrays~\cite{Xu2025}.

There are multiple ways to achieve a joint optimization. 
Commonly, a weighted sum of loss terms of the different components is employed similar to \eqref{eq:isac-tradeoffs}. 
Other options to combine loss terms include products of terms, especially if fairness or reliability are of interest, or adding penalty terms if the minimum performance of a certain component is not achieved. 
Another option especially of interest when the graph for backpropagation becomes very large is alternating or sequential optimization, where certain parameters are fixed while others are optimized, switching between different graphs and loss functions.

Specifically for \ac{ISAC} systems, \ac{RIS} have attracted a lot of interest as a new system component to increase sensing or communication coverage.
The introduction of \acp{RIS} increases the degrees of freedom for potential coverage or sensing optimization, resulting in the optimization through \ac{ML} emerging as a natural candidate to approach these problems.

The problem of channel estimation for \ac{RIS} is addressed for single users in~\cite{liu2023deep} and for multi-user configurations in~\cite{liu2023extreme}. The training data is generated through channel simulations and enriched through data augmentation. In~\cite{liu2023extreme}, an \ac{ELM}, which is a generalized type of \ac{NN} with additional trainable parameters, is used to perform the channel estimation. As uplink and downlink signals are considered, a two-stage approach is evaluated.
%The authors remain mindful of computational complexity and provide extensive simulations to evaluate the system's performance.
In~\cite{zhang2024joint}, the transmit signal optimization for an \ac{ISAC} system with \ac{RIS} is optimized, minimizing interference.
An algorithm based on the alternating direction method of multipliers is developed and made trainable through deep unfolding. Unsupervised learning is used to minimize the weighted sum of multi-user interference energy and waveform discrepancy. 
%These studies indicate that new design paradigms for wireless networks can be well suited to explore using \ac{ML}.

% \begin{itemize}
%     \item Explore new network paradigms: \textit{RIS:} channel estimation in single  and multi user \cite{liu2023extreme} ISAC scenarios. This work uses deep unfolding to optimize the transmit waveform and phase shift \cite{zhang2024joint}.  
% \end{itemize}
\subsection{Target Estimation}
%
In this section, target estimation refers to radar-like sensing, where the \ac{TX} signal is reflected passive targets, i.e., reflectors in the environment that are not wireless link endpoints (as \ac{TX} or \ac{RX}).
After the acquisition of the wireless channel estimate (see \eqref{continuous_time_channel}), the sensing signal processing must detect and estimate the propagation parameters of the unknown number of targets.
From the detected and estimated propagation parameters, geometrical targets positions, velocity, size, or orientation are estimated. 
Generally, the available propagation parameters for each target include the delay (range), Doppler-shift (relative velocity), \ac{DoA}, \ac{DoD}, and complex path weights (including polarization). 
However, measurement system capabilities impose limitations, e.g., \ac{DoA} and \ac{DoD} are only possible in multi-antenna systems.
As different systems allow for the estimation of different propagation parameter types, we discuss them separately in the following subsections, starting with the range-Doppler detection and estimation as the default case.
% The joint detection of object and parameter estimation will be covered in Sec.~\ref{}.
\subsubsection{Classical Estimation}
\todo[inline]{Add the harmonical retrieval problem, then ML estimation, CR-bounds, approach, subspace methods, compressed sensing}

\subsubsection{Angle Estimation}
As described in \eqref{continuous_time_channel_node}, when considering different RXs a waveform impinging on an antenna may yield a phase difference in the signal captured by different RXs. This phase difference is related to the angle $\theta$ which the waveform comes from. The problem of estimating $\theta$ from the received signal is commonly known as \ac{DoA} estimation.\footnote{If the objective is to estimate the angle at which a waveform is emitted by a TX, the problem is referred to as \ac{DoD} estimation. In this section, we focus on \ac{DoA} estimation for simplicity.}
Assume an array antenna as depicted in Fig.~\ref{fig:DoA_ULA_example} estimating the \ac{DoA} from $M$ targets in the environment. Consider that the targets are in the far-field region of the antenna and that each target emits a signal $s_m(t)$ from an angle $\theta_m, m=0,\ldots,M-1$. 
Starting from the model in \eqref{continuous_time_channel_node}, consider (\textit{i}) that the targets have a \ac{LoS} path with the antenna array, which means that $L(t)=1$, and (\textit{ii}) the delay from each target to the antenna array can be estimated and compensated for, which implies that $\tau_0(t) = 0$. Then, the channel model for each target is
\begin{align}
    h_i(t,\tau) = \alpha(t) \delta(t-\tau_{i,0}(t))e^{-\j 2\pi f_c \tau_{i,0}(t)}.
\end{align}
According to Fig.~\ref{fig:DoA_ULA_example}, $\tau_{i,0}(t)=id\sin(\theta(t))/c$, $i=0,\ldots,K-1$, where $d$ is the distance between RXs and $c$ is the speed of light. In the case of a narrowband signal $s(t-\tau_{i,0})\approx s(t)$.\footnote{Extensions for wideband signals have been proposed, but we skip their description for simplicity.} Following \eqref{ReceiverSignal} and considering the superposition of signals from different targets, the output signal at the $i$-th RX is
\begin{align} \label{eq:y_i(t)_angle}
    y_i(t) = \sum_{m=0}^{M-1} \alpha_m(t) s_m(t) e^{-\j 2\pi i\frac{d}{\lambda}\sin(\theta_m(t))} + n(t).
\end{align}
The continuous-time received signal in \eqref{eq:y_i(t)_angle} is sampled and  $T$ transmissions (often called \textit{snapshots}) can be collected for further processing. We assume that during the time of $T$ snapshots, the angle of the targets and the complex channel gain remain constant. Aggregating the received samples across antenna elements and snapshots, the discrete-time received signal $\bm{Y}$ can be expressed as:
\begin{align} \label{eq:rx_signal_array_doa}
    \bm{Y} = \bm{A}(\theta)\bm{S} + \bm{N},
\end{align}
where $\bm{A} = [\bm{a}(\theta_1), \ldots, \bm{a}(\theta_M)]\in\complexset[K][M]$ is a matrix containing steering vectors of the form
\begin{align}
    \bm{a}(\theta) = [1, e^{-\jmath 2 \pi d \sin{(\theta)}/\lambda}, \ldots, e^{-\j 2 \pi d (K-1) \sin{(\theta)}/\lambda}]. 
\end{align}
The sampled received signal for each target and snapshot are aggregated in $\bm{S} = [\bm{s}(1), \ldots, \bm{s}(T)]$, where the complex channel gain $\alpha_m$ is absorbed in $s_m$ and $\bm{N}$ represents the additive noise.

There are different kinds of \ac{DoA} estimation methods: (\textit{i}) \ac{MLE} methods, (\textit{ii}) subspace methods, and (\textit{iii}) \ac{CS} methods. \ac{MLE} methods attempt to solve the following optimization problem
\begin{align}
    \hat{\bm{\theta}} = \arg\max_{\bm{\theta}} \mathfrak{L}(\bm{\theta}|\bm{Y}),
\end{align}
where $\bm{\theta}=[\theta_1,\ldots,\theta_M]^\top$. The function $\mathfrak{L}(\bm{\theta}|\bm{Y})$ is the probability function of DoAs given the received signal, called the  \textit{likelihood function}. The likelihood function is in most cases multimodal, which hinders the implementation of MLE methods \cite{viberg91detection}. Several approaches have been proposed to solve this problem \cite{viberg91detection, stoica90maximum, sharman89genetic}, but they require high \ac{SNR}, large computational costs, good initial DoA estimation, or a small number of targets to estimate.

Subspace methods obtain computationally efficient algorithms compared to MLE methods~\cite{chung2014doa}. Subspace methods rely on the estimation of the covariance matrix of the received signal, defined as
\begin{align}
    \bmRY = \E[\bm{Y}\bm{Y}^{\hermit}] = \bm{A}(\theta)\bmRS \bm{A}^{\hermit}(\theta) + \bmRN,
\end{align}
where $\bmRS$ is the covariance matrix of $\bm{S}$, $\bmRN$ is the covariance matrix of $\bm{N}$, and we assumed that $\bm{N}$ is zero--mean and independent from $\bm{S}$. Since $\bmRY$ is a Hermitian symmetric matrix, the eigenvectors of $\bmRY$ are orthogonal and a eigenvalue decomposition yields
\begin{align}
    \bmRY = \bm{U}\bm{\Lambda}\bm{U}^{\hermit},
\end{align}
where $\bm{\Lambda}=\diag(\lambda_1,\ldots, \lambda_K)$ and $\bm{U}=[\bm{u}_1, \ldots, \bm{u}_K]$ contain the eigenvalues and eigenvectors of $\bmRY$, respectively. The matrix $\bm{U}$ spans a subspace that can be partitioned into two orthogonal subspaces: (\textit{i}) the signal subspace and (\textit{ii}) the noise subspace, i.e., $\bm{U} = [\bmUS|\bmUN]$, where $\bmUS$ contains the $M$ eigenvectors corresponding with the $M$ eigenvalues with largest magnitude and $\bmUN$ the remaining $K-M$ eigenvectors. Subspace methods use $\bmUS$ or $\bmUN$ to perform angle estimation, leading to methods such as \ac{MUSIC}~\cite{schmidt86multiple}, root-\ac{MUSIC}~\cite{barabell83improving}, or \ac{ESPRIT}~\cite{roy89esprit}.
Subspace methods rely on the following assumptions: (\textit{i}) the number of snapshots is large enough so that the estimated covariance matrix
\begin{align} \label{eq:est_cov_matrix}
    \hat{\bm{R}}_{\text{Y}} = \frac{1}{T} \bm{Y}\bm{Y}^{\hermit}
\end{align}
is similar to $\bmRY$, (\textit{ii}) the sources are uncorrelated so that $\bmRY$ is full rank, and (\textit{iii}) the \ac{SNR} is not low. If these conditions are not met, subspace methods degrade in performance. 
\ac{CS} methods have become more popular in recent years since they can solve the disadvantages of subspace methods \cite{shen16underdetermined, aich17ongrid}. \ac{CS} methods exploit the sparse distribution of the spatial source signals \cite{malioutov05space}. In the narrow-band, multiple-snapshot case of \eqref{eq:rx_signal_array_doa},\footnote{\ac{CS} for DoA estimation can be applied to a wideband signal model or a single snapshot, see \cite{shen16underdetermined}.} we consider a grid of candidate angles $\{\theta_{\gtext,i}\}_{i=0}^{N_g-1}$ and we construct $\bm{S}_{\gtext} = [\bm{s}_{\gtext,0},\ldots, \bm{s}_{\gtext,T}]$, where the $j$-th value of $\bm{s}_{\gtext,t}$ is nonzero if there is a target at angle $\theta_{j}$ for the $t$-th snapshot. \ac{CS} tries to solve the following optimization problem:
\begin{align} \label{eq:CS_doa_problem_0}
    \min_{\bm{S}_{\gtext}}&\ \norm{\tilde{\bm{s}}_{\gtext}}_0 \nonumber \\
    \text{s.t.}&\ \norm{\bar{\bm{y}} - \bm{A}(\bm{\theta}_{\gtext})\bar{\bm{s}}_{\gtext}}_2 \leq \varepsilon,
\end{align}
where $\tilde{\bm{s}}_{\gtext}$ is computed by taking the $l_2$ norm to each row of $\bm{S}_{\gtext}$, $\norm{\cdot}_0$ is the $l_0$ norm, $\bar{\bm{y}} = \vectext(\bm{Y})$, $\bar{\bm{s}}_{\gtext} = \vectext(\bm{S}_{\gtext})$, and $\norm{\cdot}_2$ is the $l_2$ norm. The problem in \eqref{eq:CS_doa_problem_0} is difficult to solve, and the $l_1$ norm is used as an approximation \cite{candes06robust}. Examples of \ac{CS}-based algorithms are basis pursuit \cite{chen94basis}, \ac{OMP} \cite{mallat93matching}, and sparse Bayesian learning \cite{tipping2001sparse, wipf04sparse}, among others.
The disadvantages of \ac{CS} methods are that (\textit{i}) they are more computationally complex than subspace methods since the matrix $\bm{S}_{\gtext}$ is larger than $\bmRY$ and (\textit{ii}) iterative algorithms such as OMP can propagate errors if the estimations are not correct in the first iterations.
Moreover, a common assumption of all \ac{DoA} estimation methods is that the model of \eqref{eq:rx_signal_array_doa} holds. Under hardware impairments, methods degrade in performance due to model mismatch.
In this context, \ac{ML} can be harnessed to reduce the complexity of \ac{CS} methods or to improve the estimation of subspace methods under few snapshots, coherent sources, low SNRs and modeling mismatches like broadband signals or hardware impairments. A first natural step to \ac{DoA} estimation using deep learning is to use the received signal $\bm{Y}$ as input to a \ac{NN} and obtain the \ac{DoA} as output, i.e., following the notation of Sec.~\ref{sec:ml-basics},
\begin{align} \label{eq:theta_output_Y_doa}
	\hat{\theta} = f(\bm{Y};\mat{\Theta}).
\end{align} 
To improve the angular resolution of the estimated \ac{DoA}, the field-of-view of the receive antenna is discretized in angular candidates $\{\theta_i\}_{i=1}^N$ and the output of the \ac{NN} is a probability vector that represents the probability that each angular candidate is the true angle, i.e., 
\begin{align} \label{eq:p_output_Y_doa}
    \hat{\theta} = \sum_{i=1}^K \theta_i \hat{\bm{p}}_i,
\end{align}
with $\hat{\bm{p}} = f(\bm{Y};\mat{\Theta})$. This can be achieved using a softmax layer as output layer of the NN. The \ac{DoA} estimation problem is regarded as a multi-class classification problem and the categorical \ac{CE} loss is used to train the \ac{NN} \cite{zheng2024deep}. An extension of this approach is to discretize a smaller angular sector instead of the entire field-of-view, which provides a more accurate angular estimation \cite{ma2022deep}. A similar way to consider a discrete angular grid as output to the NN is to compute the spatial spectrum, defined as $|\bm{a}^T(\theta)\hat{\bm{p}}|$ for different values of $\theta$. The estimated spatial spectrum computed from $\hat{\bm{p}}$ can be compared with the true spatial spectrum from the true \ac{DoA} \cite{chen2024sdoa}. Inspired by the subspace methods, an estimate of the covariance matrix can be used as input to the NN. However, the covariance matrix is Hermitian by the definition in \eqref{eq:est_cov_matrix}. Thus, the upper triangular part of $\bmRY$ contains all the information about $\bmRY$ and can be used instead of the entire covariance matrix. One approach is to use a vectorized and normalized version of the covariance matrix as input to a MLP \cite{zhu2020two}, i.e., 
\begin{align}
    \bm{r} = [&\mathcal{R}\{{\bm{R}_{1,2}}\}, \mathcal{I}\{{\bm{R}_{1,2}}\}, \mathcal{R}\{{\bm{R}_{1,3}}\}, \mathcal{I}\{{\bm{R}_{1,3}}\}, \ldots, \\ \nonumber
    &\mathcal{R}\{{\bm{R}_{N,N}}\}, \mathcal{I}\{{\bm{R}_{N,N}}\}].
\end{align}
The input to a MLP can be $\bm{v} = \bm{r}/\lVert \bm{r} \rVert^2$ \cite{chen2022robust}. Moreover, the vector $\bm{v}$ can be reshaped back to a matrix and use a CNN to process the covariance matrix. The output of the CNN can be the same as in \eqref{eq:theta_output_Y_doa} or \eqref{eq:p_output_Y_doa} \cite{chen2022robust, yu2023deep}.
Most of the limitations of subspace methods stem from the fact that the estimated covariance matrix is not similar to the true covariance matrix. However, under a good estimation of the covariance matrix, subspace methods obtain good performance. This idea is the basis of \ac{MBL} for DoA estimation. In the case of DoA estimation, $h_{\bm{\theta}}$ in \eqref{eq:mbl} can be a CNN that takes the estimated covariance matrix (or its upper-triangular part) as input and produces another matrix as output that can be used by root-MUSIC to estimate the DoA  \cite{shmuel2023subspacenet}. The output matrix can also be processed to compute the MUSIC spectrum and then a MLP yields the estimated DoA \cite{merkofer2024damusic}. 
A further step in \ac{MBL} is to learn just the parameters that affect the performance of subspace methods instead of using DNNs. In particular, for the case of hardware impairments, learning the parameters subject to impairments allows to calibrate the system. For instance, considering gain and position impairments in the ULA, the impaired steering vector becomes 
\begin{equation} \label{eq:impaired_steer_vector}
	[\bm{\tilde{a}}(\theta)]_k = g_k e^{\jmath 2 \pi p_k \sin(\theta)}, 
\end{equation}
where $g_k$ and $p_k$ are the unknown gains and positions of the elements of the ULA. Considering as learnable parameters $\mat{\Theta} = \{g_k, p_k\}_{k=1}^K$ and using a subspace method that enables backpropagation, the performance of the impaired system can be improved \cite{chatelier2025physically}.   
As a summary, in Table~\ref{tab:DoA_estimation}, we collect the most recent DoA estimation works, highlighting the problems from classical DoA estimation that they address. 
%The most recent studies \cite{shmuel2023subspacenet, merkofer2024damusic} show that \ac{MBL} methods that enhance subspace methods can account for all the mismatched assumptions of subspace methods with lower complexity than \ac{CS} methods.

\begin{comment}
    
\begin{itemize}
	\item \cite{ma2022deep} uses a single snapshot, the raw received signal as input to the NN, and the problem is treated as a multi-class classification problem. They consider a narrow angular sector $[-\phi, \phi]$ divided into $K$ grids. Considering a binary decision for each of the $K$ grid points, there are $2^K$ combinations of targets. They consider a softmax output layer with a size of $2^K$. This is the central idea, but they also require further processing of the received signal to take any angular sector to the central region $[-\phi, \phi]$.
	\item \cite{zheng2024deep}  uses the raw received signal as input, but concatenates the real and imag. parts  in a different way (maybe \cite{ma2022deep} concatenates data in a different way). They propose a classification and a regression model. They also consider a grid of points for the angular sector.
	\item \cite{chen2024sdoa} considers multiple snapshots. The input to the NN is the raw received signal, divided into real and imaginary part (concatenated vertically). The output of the NN is a vector that is used to compute the "spatial spectrum". The estimated spatial spectrum is compared with the "true" one, which is a mixture of Gaussian models.

	\item \cite{zhu2020two} considers a UCA. The input to the CNN is the upper-trian. cov. matrix after it has been vectorized and normalized. The output consists of 4 neurons: one for the azimuth angle two for the sin and cos of the azimuth (?) and one for the elevation angle. They also consider an ensemble of DNNs to improve performance.
	\item \cite{yu2023deep} considers a uniform planar array instead of a ULA. They consider a single snapshot. They use as input to the CNN a processed version of the upper triangular part of the covariance matrix. They consider 3 CNNs: (i) that estimates the number of paths including LoS, (ii) estimates the DoA of the LoS path, and (iii) estimates de Doa of the NLoS paths. All CNNs use a processed version of the cov. matrix, but it is unclear how the CNNs interact.
	\item \cite{chen2022robust} They use multiple snapshots. This work is also suitable for low SNR, I should include that on the table. The input to the NN is the upper-triangular part of the covariance matrix w/o the diagonal elements. The output of a first NN are some functions that depend on different angle grid point that cover the entire space (this is not very clear how it's done). 

	
	\item \cite{shmuel2023subspacenet} takes as input an estimate of the covariance matrix (but averaged over different lags) and produces as output a matrix that futher processed (to be hermitian symmetric) yields the cov. matrix to be used by subspace methods.
	\item \cite{merkofer2024damusic} uses multiple snapshots (but maybe it also shows robustness against fewer snapshots?), and an architecture with multiple NNs (see Fig. 3). It takes the input signal to a GRU to compute a covariance matrix, then they apply EVD to obtain the MUSIC spectrum, which is the input to another NN to estimate the angle of the targets. This is the core idea, and more processing is needed if the number of sources in unknonwn. To train the model, the root mean squared periodic error is used, where all combinations of true/estimated targets are considered.
	
	\item \cite{chatelier2025physically} Considers multiple snapshots. They learn the gain and position impairments deriving a differentiable MUSIC algorithm. 
	
	
	\item \cite{labbaf2023robust} They consider UCA, multiple snapshots. The input to the NN arquitecture is the cov. matrix but only the upper triangular part because it's Hermitian symmetric. I'm tempted to rule out this paper as well because the NN architecture is unclear.
	\item \cite{muth2024loss} uses multiple snapshots and the cov. matrix as input to a MLP perceptron. Maybe I remove it from here since it's already mentioned in the prev. section.
	\item \cite{ahmed2021deep} is going to be removed from the list.
	\item \cite{hu2020low} considers a single snapshot and a UCA. I'm tempted to remove this, because they use D NNs to have candidate angles and then they solve a max. likeli. problem by grid search, but it's unclear how they make it differentiable and how they assure the candidate angles are not the same or they cover the entire angular space. 
\end{itemize}
\end{comment}

\begin{table*}[tb]
\centering
\renewcommand{\arraystretch}{1.2} % Adjust row spacing
\caption{ML-based DoA estimation works.}
\label{tab:DoA_estimation}
\begin{tabular}{l|l|l|l|l|l|l|l|l}
\hline\hline
 & Ref. & ML method & \begin{tabular}[c]{@{}l@{}}Low \\ SNR\end{tabular} & \begin{tabular}[c]{@{}l@{}}Few\\ Snapshots\end{tabular} & \begin{tabular}[c]{@{}l@{}}Complexity \\ reduction\end{tabular} & \begin{tabular}[c]{@{}l@{}}Hardware \\ impairments\end{tabular} & \begin{tabular}[c]{@{}l@{}}Coherent \\ sources\end{tabular} & \begin{tabular}[c]{@{}l@{}}Broad-band\\ signals\end{tabular} \\ \hline
\multirow{8}{*}{DL} 
 & \cite{zheng2024deep} & CNN & \checkmark & \checkmark &  &  &  &  \\\cline{2-9}
 & \cite{ma2022deep} & CNN &  & \checkmark &  &  &  &  \\
 \cline{2-9}
 & \cite{chen2024sdoa} & CNN &  &  & \checkmark  & \checkmark &  &  \\
 \cline{2-9}
 & \cite{zhu2020two} & Ensemble DL &  &  & \checkmark &  &  &  \\\cline{2-9}
  & \cite{chen2022robust} & \begin{tabular}[c]{@{}l@{}}Denoising\\ autoencoder\end{tabular} &  &  &  & \checkmark &  &  \\ \cline{2-9}
   & \cite{yu2023deep} & CNN & \checkmark &  &  &  &  &  \\ 
\hline
\multirow{4}{*}{MBL} & \cite{shmuel2023subspacenet} & \begin{tabular}[c]{@{}l@{}}Data-augmented\\ root-MUSIC\end{tabular} & 
 \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\ \cline{2-9}
 & \cite{merkofer2024damusic} & \begin{tabular}[c]{@{}l@{}}Data-augmented\\ MUSIC\end{tabular} & \checkmark  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\ \cline{2-9}
 & \cite{chatelier2025physically} & \begin{tabular}[c]{@{}l@{}}Data-augmented\\ MUSIC\end{tabular} &   &  &  & \checkmark &  &  \\
 \hline\hline
\end{tabular}
\end{table*}

\subsubsection{Joint Range-Doppler Detection and Estimation}
Target detection refers to the decision-making of if or how many targets are present in a certain area of interest. This is commonly done based on the \ac{RDM}, where the channel is described by the 2D power profile over delay (or range) and frequency, exemplified in Fig. \ref{fig:periodogram}. Clasically, detection is performed by a variation of \ac{CFAR} detector. The \ac{RDM} is commonly calculated using a series of frequency responses as defined in~\eqref{discrete_frequency_channel}. The detection problem is a peak detection issue at its core, yet extracting the targets from the \ac{RDM} can become difficult in reality. 

For an \ac{OFDM} waveform, the \ac{RDM} is commonly calculated by concatenating a series of $M$ transmit and receive OFDM symbols after removal of the cyclic prefix to the frames $\mat{X}\in \mathbb{C}^{K\times M}$ and $\mat{R}\in \mathbb{C}^{K\times M}$, respectively. $M$ channel estimates in frequency domain akin to \eqref{discrete_frequency_channel} are obtained by a elementwise division of $\mat{R}$ and $\mat{X}$. 
Then the \ac{RDM} is
\begin{align} \label{eq:rdm}
    \mathrm{RDM} =  \bm{F}^*_K \left(\mat{R} \oslash \mat{X} \right)  \bm{F}_M^{\top},
\end{align}
with $\bm{F}_N$ the $N$-point DFT unitary matrix. We perform a column-wise IFFT to transform from the frequency into delay domain and a row-wise FFT to transform from time into Doppler domain. 

A statistically optimal detector in \ac{AWGN} is a Neyman-Pearson detector, that tests if at the estimate of the channel $\hat{h}$ at the discrete time delay $n$ a target is present, can be formulated as~\cite[Chap. 10]{Trees2002}:
\begin{align}
    \frac{2}{\sigma_{\text{n}}^2} |\hat{h}_{n}|^2 \quad\mathop{\gtreqless}_{\hat{T}=0}^{\hat{T}=1}\quad \chi^2_{2}(1-P_{\text{f}}),
\end{align}
where $\chi^2_{2}(\cdot)$ denotes the chi-squared distribution with $2$ degrees of freedom, $P_{\text{f}}$ is the false alarm rate of detection and $\sigma_{\text{n}}^2$ denotes the noise power.
In more sophisticated scenarios with extended targets, sidelobes and clutter a more practical cell-averaging \ac{CFAR} (CA-CFAR) approach is usually taken that does not need an implicit estimate of the noise. 

Additional filtering can be applied depending on the transmit signal and/or expected shape of targets, as preprocessing or as a dedicated part of a modified CA-CFAR algorithm.
The radar image does not only show the target reflections, but is also influenced by distortions caused by the transmit signal structure, clutter, or ghost targets, which can be very challenging to address with classical approaches. Additionally, it can be challenging to differentiate between closely spaced targets. CA-CFAR and its variants estimate the noise from neighboring channel estimates, which can be difficult if other targets are inside these neighboring channel estimates.
\begin{figure}[t]
    \def\mathdefault#1{#1}
    \begin{center}
        \scalebox{0.85}{
    \input{figures/periodogram/periodogram.pgf}}
    \end{center}
    \caption{\ac{RDM} of an \ac{ISAC} measurement. Sidelobes and clutter are present which can inhibit efficient target detection and estimation.}
    \label{fig:periodogram}
\end{figure}
Detection and localization can also be performed in tandem, if a detection hypothesis is tested for multiple different positions in the illuminated area.
For classical algorithms, it can be challenging to consider specific observation areas, without discarding detections outside the area of interest. Removing clutter from the sensing environment, leading to false alarm detections, is an additional challenge. Lastly, the distinct geometry or micro-Doppler of targets, affecting the distinct pattern associated with the target in the \ac{RDM}, can be used to increase the detection accuracy. Yet, with classical algorithms, these are difficult to model accurately for filtering purposes.
In contrast, trainable algorithms can get better detection rates under the same false alarm rate if they are trained to take the area of interest, including its clutter or the characteristic features of the targets into account, which can be included in the training data.

In~\cite{Dong2024}, the features of space debris targets are used to detect them. The study combines support vector machines and \ac{CSI}-based sensing. The algorithm is trained based on simulated scenarios and measurement data to achieve accurate detection and classification of the type of debris.
In~\cite{muth2023autoencoder} considering multiple targets and~\cite{muth2024loss} considering multiple snapshots, the comparison with a trainable detector and a classical statistical detector is performed. It is shown using simulations that we can overcome the performance of generally optimal detectors while staying at the same false alarm rate. This is possible because the training data contains typical features of the scenario, e.g. a specified area of interest.

In the radar community, The detection problem has also been considered. In~\cite{jiang2019end}, the waveform and detector are trained to approach a Neyman-Pearson detector, which is optimal in white noise. While no a priori information about the target and clutter model is assumed, the trained solution achieves a more robust detection rate compared to classical solutions in clutter and colored noise.
In~\cite{major2019vehicle}, deep learning is used to differentiate targets such as vehicles from clutter based on the \ac{RDM}. This work underlines how detection and object classification can often be entwined, as in measurements some type of clutter is to be expected.

\subsubsection{Delay/Range-Doppler Estimation}
Estimating the range and Doppler-shift of the detected targets enables the determination of a target’s range and relative radial velocity. 
Typical algorithms include using peak positions from the \ac{RDM}, subspace methods like \ac{ESPRIT}, \ac{CS}, and \ac{MLE} approaches.
In general, they leverage the algebraic structure of the signal model (see \eqref{continuous_time_channel}), which shares its structure with multidimensional harmonic retrieval and are therefore also algebraically similar to angular estimation techniques.

However, conventional methods are affected by imperfections arising from non-ideal measurement hardware effects, such as non-linearities, quantization, and imperfect calibration.
Such mismatches degrade the performance of algorithms reliant on the idealized signal models.
While \ac{ML}-methods are affected similarly (depending on how they are trained), they can be used to alleviate the adverse effects.
For example, \cite{shmuel2023subspacenet} demonstrates SubspaceNet, an approach to mitigate the effects of imperfect antenna array calibration on subspace-methods.
To this end, they combine a deep autoencoder with a RootMUSIC estimator during the training, which enables backpropagation. 
The results show that the autoencoder is not just able to adapt the mismatched data to improve the RootMUSIC performance, but also improves the performance when applied with \ac{ESPRIT}.
Comparably, \cite{schielerCNNMeasurement} also demonstrates that it is possible to train a \ac{CNN} for estimation on synthetic data and transfer it to measurement data, alleviating the need for costly measurement data collection.

Another issue is presented by extended targets, which appear as a superposition of insufficiently separated paths (in terms of sampling resolution) to an estimator based on \eqref{continuous_time_channel}. 
As a consequence, these paths create an additional overhead in the estimation, and leveraging them for classification requires additional hand-designed algorithms. 
Comparably, they present an opportunity for \ac{ML} approaches, which can leverage the characteristic shape of the target to reduce the number of false alarms and/or perform simple target classification (e.g., whether there is a target and whether or not it contains micro-doppler).

Beyond robustness, computational complexity poses another challenge. 
Iterative \ac{MLE} estimators like RIMAX \cite{richterEstimation2005} achieve high accuracy but at significant computational cost, which is challenging to reduce~\cite{semper2024}. 
Both \cite{Barthelme2021} and \cite{schielerGridFree2024} present approaches to alleviate this computational cost by combining conventional \ac{MLE} methods with \ac{ML}.
They illustrate that \acp{NN} can effectively initialize gradient-based \ac{MLE} methods, reducing runtime while maintaining accuracy. 
These hybrid approaches combine the efficiency of data-driven methods with the precision of model-based optimization, circumventing the need for exhaustive iterative searches.

\subsubsection{Angle-Range Estimation}
The position of a target can be estimated transmitting a signal that contains different frequency components and using the same signal for different antenna elements. At the \ac{RX} side, an \textit{angle-range} matrix can be computed from the received signal across antenna elements and frequencies similarly to the RDM of \eqref{eq:rdm}. 
\Ac{ML} has been used in angle-range estimation to compensate for hardware impairments. Particularly, \ac{MBL} was harnessed in \cite{mateos2024model} to compensate for hardware impairments while performing angle-range estimation and target detection. The considered impairments are inter-antenna spacing impairments, similarly to \eqref{eq:impaired_steer_vector} and the learnable parameters are the positions of the antenna elements in the \ac{ULA}. In Fig.~\ref{fig:results_angle_range}, sensing results are represented as a function of the false alarm rate for the multi-target scenario of \cite{mateos2024model}. The MBL approach is compared with the baseline with perfect knowledge of the impairments and with a model-based calibration technique that requires no gradient backpropagation. Fig.~\ref{fig:results_angle_range} suggests that with MBL the performance of the system without impairments can be closely approached and with MBL the performance of model-based calibration can be outperformed.  
This work was extended in \cite{mateos2024semi} to reduce the amount of labeled data by designing an unsupervised loss function.

\begin{figure}[tb]
    \centering
    \includestandalone[width=0.4\textwidth]{figures/ISAC/angle-range/results}
    \caption{Position error as a function of the false alarm rate. The results are computed from synthesized data considering a MIMO-OFDM radar with 64 antenna elements and 256 subcarriers. A maximum number of 5 targets in the scene are assumed, considering a random number in each snapshot. Inter-antenna spacing impairments were considered in the ISAC transceiver.} 
    \label{fig:results_angle_range}
\end{figure}

% \subsubsection{Range-Doppler Estimation:}
% Joint target detection and parameter estimation with a \ac{CNN} from frequency and time samples of a radio channel's transfer function has recently been proposed by \cite{schielerGridFree2024}. 
% Instead of using a \ac{CFAR} detector with a different subsequent estimation algorithms as commonly done in radar sensing, \cite{schielerGridFree2024} demonstrates the use of a \ac{CNN} for joint detection and estimation.

% The authors propose a Convolutional Neural Network (CNN) architecture designed to jointly estimate the number of targets (model order) and their corresponding parameters in a quasi-grid-free manner, such that off-grid estimates are attainable. 
% Doing so mitigates issues inherent in grid-based methods, such as bias, spectral leakage, and the detection of spurious components (ghost targets). 
% A key innovation is the multi-channel windowing technique applied during data preprocessing, which enhances the estimator's robustness and can be considered a trainable version of multitaper analysis \cite{thomsonSpectrum1982}. 
% It therefore presenting a deep learning framework that effectively combines target detection and estimation offering advantages over conventional grid-based methods.

% Additionally the approach can be combined with a gradient-based maximum-likelihood estimator.
% The estimates from the \ac{CNN} are used as initial values for a subsequent gradient-based optimization algorithm, whose estimates achieve the \ac{CRB}.
% Instead of iterative initialization, the computational complexity of the global search procedure in iterative maximum-likelihood estimators, such as RIMAX \cite{richterEstimation2005}, is reduced by intializing multiple targets at once, which greatly reduces the overall number of iterations.

% The approach presents a form of Physics-informed machine learning (see~\cite{karniadakisPhysicsInformed2021}) through the strong integration of physical propagation- and signal models into the preprocessing, CNN architecture, and training data generation. 
% As the approach is trained solely on synthetic data, generated from a suitable model of the physical propagation such as \ref{discrete_frequency_channel}, it does not require costly collection and labeling of measurement data.
% Prior knowledge, e.g., of site-specific propagation characteristics from channel models, can be incorporated into the training process to improve performance for the specific scenario.

\subsubsection{Range-Angle-Doppler Estimation}
Range-Angle-Doppler (RAD) estimation is a fundamental part of advanced driving assistance systems (ADAS).  
Light detection and ranging (LIDAR) is commonly used in ADAS since it is lightweight, cost-effective, and precise. However, the operation of LIDAR is severely affected by adverse weather conditions, e.g., fog, snow, or heavy rain. Conversely, mmWave radar is more robust under harsh conditions at the expense of sparser clouds of points to detect targets. 
To improve the performance of mmWave radar for RAD estimation, in \cite{hu2023radnet} the accuracy of existing standard processing methods was improved with DL. Another use case of \ac{ML} in RAD estimation is to improve the resilience of the estimation against jamming. Jamming refers to the intentional malfunction of a receiver by sending interfering signals. In \cite{Benyahia2022squeeze}, ML is harnessed to improve RAD estimation against clutter and jamming.

\subsection{Tracking}
So far, we have considered that we obtain an estimate of the target position and velocity every time that one or multiple snapshots were transmitted. These estimates over time form the trajectory of each target in the scene. If target trajectories are considered instead of independent estimates, the estimate of the target position and velocity in the next time step can be improved. Tracking refers to the estimation of the trajectory of targets in the scene.
However, the major challenge of tracking is to associate new measurements with object trajectories including: (\textit{i}) creating new trajectories, (\textit{ii}) removing existing trajectories, and (\textit{iii}) distinguishing clutter from targets. 
%%% In Fig.~\ref{fig:trajectories}, there is an example of the estimated position of different objects in a scene. From all the measurements, the trajectories of each target should be estimated. 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/ISAC/tracking/trajectories.pdf}
%     \caption{Example of tracking three targets in a scene. Lighter colors mean earlier measurements.}
%     \label{fig:trajectories}
% \end{figure}
There have been several algorithms proposed for multi-object tracking, such as the probability hypothesis density~\cite{garcia19trajectory}, the generalized labeled multi-Bernoulli~\cite{vo19multi}, and the multi-scan trajectory Poisson multi-Bernoulli mixture~\cite{xia2019multi}. However, the unknown measurement-target association makes these approaches have a super-exponential complexity in the number of time steps to process~\cite{mahler2007statistical}.
\Ac{ML} can reduce the computational complexity of conventional tracking algorithms.
At the transmitter side, tracking is used to predict the user position and perform beamforming, which can help in the design of narrower beams with larger antenna arrays to increase the data rate of users. Predictive and adaptive beamforming was studied in \cite{liu2022learning}, where an unsupervised approach with an \ac{LSTM} network is proposed. 
The work in \cite{wang2023deep} also uses an \ac{LSTM} network with the raw data instead of a two-step approach where the positions of targets are estimated and then beamforming is performed. Strategies to reduce training overhead have also been proposed \cite{demirhan2022radar}.
At the \ac{RX} side, multi-object tracking was addressed with a tailored transformer in \cite{pinto2023deep}. \Ac{MBL} solutions have also been developed based on the Kalman filter. The Kalman filter provides the \ac{MMSE} estimator for a time-varying discrete system under \ac{AWGN}. It is based on linear equations that describe how the system evolves over time, referred to as the state-space model. However, many problems involve non-linear state-space models. Several solutions have been proposed, such as the extended Kalman filter \cite{gruber1967approach} and the unscented Kalman filter \cite{julier1997new}. The family of particle filters \cite{gordon1993novel, del1997nonlinear} was also introduced for non-linear, non-Gaussian state space models, which obtains better results than the Kalman filter with higher computational complexity. 
The main weakness of the aforementioned filters is that they rely on the state-space model and filters exhibit performance degradation if the state-space model is not accurate. Several works deal with some level of uncertainty in the state-space model, but they cannot achieve the same performance as the filters with full knowledge.
\ac{MBL} methods can enhance conventional filters to adapt to unexpected deviations from the assumed state-space models. Regarding the Kalman filter, the work in \cite{revach2022kalmannet} augments the Kalman filter to deal with non-linearities and model mismatches. This approach was extended to make the \ac{NN} robust against changes in the model \cite{ni2024adaptive} or to quantify the uncertainty in the estimations by extracting the error covariance matrix \cite{dahan2024uncertainty}. The particle filter was also augmented with DL to mitigate model mismatch~\cite{nuri2024learning}.

\subsection{State Detection and Object Classification}
Apart from the position and velocity of targets estimated in previous sections, targets possess other useful features to be estimated. For instance, the type of target (pedestrian, bike, car) and their size can be used in ADAS or the actions of a person are useful to monitor in eHealth applications. In this section, we consider the estimation of target features different from their position and velocity.

\subsubsection{Target Size Estimation}
Detecting targets and their size in a scene has typically been addressed by computer vision techniques from camera measurements~\cite{zou23object}, with a focus on 2D images. However, 3D object detection from camera images is a very challenging problem, although some progress has been made~\cite{wang2019pseudo}. In terms of only radar measurements, the problem of estimating the size of an object becomes even more challenging due to clutter. ML can be used to solve such complex tasks. For instance, in \cite{dong2020probabilistic}, targets are detected from \ac{FMCW} radar measurements, including their size and orientation. In \cite{ulrich2022improved}, a similar approach is done but using cloud points instead of the bird's eye view projection of the point cloud.

\subsubsection{Target Classification}
Traditional target classification only involves a small set of classes to choose from~\cite{zyweck96radar, sorowka15pedestrian}, and much attention was paid to \ac{AI} given its successful classification of images from a large number of classes. Although \ac{AI} models have excelled in image classification tasks, they have also been applied to distinguish between different kinds of targets from radar signal, involving three classes in~\cite{gupta2021target}, four classes in~\cite{ulrich2021deep}, and six classes in \cite{patel2019deep}.

% \begin{itemize}
%     \item In \cite{patel2019deep}, the authors embed a CNN in a traditional radar signal processing pipeline to classify between: 
%      construction barrier, motorbike, baby carriage, car, bicycle, and stop sign.
%     \item The authors of \cite{ulrich2021deep} use a CNN to distinguish between: car, pedestrian, cyclic and non-obstacle.
%     \item In \cite{gupta2021target}, the authors use a CNN to perform object classification between: car, human and UAV. 
% \end{itemize}


\subsubsection{Gesture Recognition}
Gesture recognition is one of the most important aspects of human-computer interaction, with applications such as developing aids for the hearing impaired, monitoring of a patient's emotional state, or lie detection~\cite{mitra07gesture}. At first, gesture recognition was based on visual aids~\cite{na19deep} or wearable sensors \cite{mukhopadhyay15wearable}. However, these sensors exhibit issues under inappropriate light conditions and they may be inconvenient to carry. The use of radar signals is robust against light conditions and users do not need to carry sensors. Among gesture recognition algorithms with radar signals, model-based algorithms rely on wave propagation theory and statistical models, requiring hand-crafted feature extraction~\cite{qi2023resource}. AI can combine feature extraction and classification and be trained to jointly optimize both tasks. Gesture recognition under the lens of AI was firstly considered using synthetic data. The work in \cite{qi2023resource} performs simulations with publicly available datasets and in \cite{du2020three}, the radar echoes are first transformed into a range-Doppler time points, which are further processed by DL. In addition, AI has also been successfully deployed in practical implementations. In \cite{bhat2023gesture}, mmWave access points were used to perform gesture recognition and in \cite{zhao2022angle}, the authors use a 4D imaging radar ---a type of radar that can measure elevation, azimuth, range, and Doppler of targets--- to classify between different human postures.

%(Charlotte)
\subsection{Environmental Sensing}
Environmental sensing refers to sensing applications, where the material parameters or a particle distribution in the air is measured instead of estimating geometrical features. An early example is radar for weather forecasting which has been in commercial deployment since the 1950s. With different bandwidths available and digital twins becoming more accessible, additional environmental features could be sensed. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/spatial_sens/neural_materials_rc_annotated.pdf}
    \caption{Learned materials from~\cite{Hoydis2023a} to obtain fine our rough representation of the environment. This graphic is under \faCreativeCommons\ \faCreativeCommonsBy CC-BY 4.0 International license }
    \label{fig:material-sensing}
\end{figure}

A more recent example for weather prediction is~\cite{bouget2021fusion}, which fuses radar images and wind forecasts using a \ac{NN} to classify between different weather classes. The open MeteoNet dataset is used for training with a \ac{CE} loss function. In comparison to a classical optical flow benchmark, more accurate predictions are achieved. In~\cite{aidin2021deep}, the rain fade for satellite communications is predicted using deep learning from satellite radar imagery as well as link power measurements. A \ac{CNN} structure processes the input data to a single output indicating the probability of rain fade.
For weather data in general, there are multiple different sensor types available, so data fusion including radar data is well established for this community. An \ac{ISAC} system with similar bandwidth and carrier frequency is potentially able to provide similar data and enhance weather prediction services.

Concerning material parameter sensing,~\cite{Helal2022} gives an overview of machine learning algorithms for terahertz sensing, which is proposed as a suited method to measure material parameters and gaseous parameters of interest. Terahertz sensing poses its own specific challenges, not only in hardware at the border of high-frequency electronics and optical systems but also for signal pre-processing, feature extraction and classification.
Lastly, in~\cite{Hoydis2023a} parameter sensing based on a known geometry is proposed as a way to improve the accuracy of virtual twins. Through raytracing, channels very accurate to the actual environment are to be simulated, yet it is unclear how much detail needs to be provided when rebuilding environments and materials. In Fig.~\ref{fig:material-sensing}, a hallway is shown with the measured reflectivity of the walls, floor and ceiling.  Depending on the complexity of the targeted material model, the radiation environment can be approximated with few materials or on a fine grid. 
% \begin{itemize}
%     \item material parameter sensing
%     \begin{itemize}
%         \item Through e.g. terahertz sensing~\cite{Helal2022}
%         \item Or with known geometry~\cite{Hoydis2023a}, improving the accuracy of virtual twins
%     \end{itemize}
%     \item rain radar, air particles...
%     \begin{itemize}
%         \item Rain prediction using rain radar images and wind forecasts \cite{bouget2021fusion}.
%         \item Rain fade prediction for satellite communications \cite{aidin2021deep}.
%     \end{itemize}
% \end{itemize}
%(Charlotte)
\subsection{Distributed Sensing}
Distributed sensing is generally of interest, as the 6G network might provide many sensing nodes. Relaying the full sensing frames to a central node might be intractable, as it results in a large signaling overhead. Therefore, we consider distributed sensing to be a sensor fusion task, where estimates from multiple nodes are fused, handled by higher layers of the communication network. The problem of distributed sensing is twofold: A representation of sensing data has to be found that can be communicated without much overhead and then a fusion algorithm has to be developed that allows estimating the result for the sensing task at hand.
This algorithm could include fusing different \ac{ISAC} nodes, different \ac{ISAC} frequency bands, or even additional sensors such as cameras or LIDAR. Concepts such as multimodal fusion using machine learning are proposed in~\cite{AI_ISAC_2024}.
As of the current knowledge of the authors, distributed sensing in the sense of fusing different \ac{ISAC} nodes hasn't manifested itself as a task clearly benefiting from \ac{AI} methods in the research literature. Many studies use classical fusion methods, but for more difficult scenarios \ac{ML} is investigated~\cite{Zhuang2023}.
In the general data fusion literature, \ac{ML} is a common tool to design performative algorithms~\cite{MENG2020115}.

% \begin{itemize}
%     \item 
%     \item 
%     \item Adjacent concepts such as multimodal fusion~\cite{10663823} have been discussed
%     \item 
%     \item data fusion problem -> not focus of this work, give some reference~\cite{MENG2020115}
% \end{itemize}

% \subsection{Questions}
% \begin{itemize}
%     \item Relevance of resource allocation -> avoid? maybe in setup/formula section
%     \item Overview: how fundamental do we want/need to go? (channel-centric, generic tx and rx)
%     \item Add section with AI/ML overview (from feed-forward networks to transformers...+ model-based learning (done sec. 1)\cite{shlezinger2023model})
%     \item Security (should be covered by open6ghub paper) jamming - spectrum sensing. (Apparently this paper will only exist as a white paper even though there was a plan to convert it into a peer-reviewed conference p.)
%     \item ignore waveforms and focus on OFDM ISAC
%     \item section before spatial sensing: introduce ISAC to make a good transition 
%     \item Should sensor fusion (e.g. with lidar) be addressed? to what depth?
% \end{itemize}
